Sense Embeddings are also Biased--Evaluating Social Biases in Static and Contextualised Sense Embeddings

Sense embedding learning methods learn different embeddings for the different senses of an ambiguous word. One sense of an ambiguous word might be socially biased while its other senses remain unbiased. In comparison to the numerous prior work evaluating the social biases in pretrained word embeddings, the biases in sense embeddings have been relatively understudied. We create a benchmark dataset for evaluating the social biases in sense embeddings and propose novel sense-specific bias evaluation measures. We conduct an extensive evaluation of multiple static and contextualised sense embeddings for various types of social biases using the proposed measures. Our experimental results show that even in cases where no biases are found at word-level, there still exist worrying levels of social biases at sense-level, which are often ignored by the word-level bias evaluation measures.

==> obsolete-related-work.tex <==
\section{Related Work}
\label{sec:related}
% To the best of our knowledge, the first and only prior work that showed that sense embeddings can also contain social biases is by \newcite{loureiro2019language}

\subsection{Sense Embeddings}

We evaluate current state-of-the-art static sense embeddings which contain social biases: LMMS~\newcite{loureiro2019language}, ARES~\newcite{scarlini2020more}. 

\subsection{Bias in Embeddings}
We focus on methods and benchmarks for evaluating bias in static and contextualised embeddings in this section.
Therefore, we do not discuss previous method to mitigate social biases.
For details on debiasing methods see~\cite{kaneko-bollegala-2019-gender,Kaneko:EACL:2021b,Kaneko:EACL:2021b,DBLP:conf/acl/RavfogelEGTG20,Dev:2019,schick2020self,wang2020doublehard}.

\paragraph{Static Embeddings:}

The Word Embedding Association Test~\cite[\textbf{WEAT};][]{WEAT} evaluates the association between two sets of target concepts (e.g. Male vs. Female) and two sets of attributes (e.g. Pleasant (\emph{love, cheer,}) vs. Unpleasant (\emph{ugly, evil}) attributes).
Here, the association is measured using the cosine similarity between word embeddings.
\newcite{ethayarajh-etal-2019-understanding} showed that WEAT systematically overestimates biases and proposed relational inner product association (\textbf{RIPA}), a subspace projection method, to overcome this problem.
Word Association Test~\cite[\textbf{WAT};][]{du-etal-2019-exploring} calculates a gender information vector for each word in an association graph~\cite{Deyne2019TheW} by propagating~\cite{Zhou2003LearningWL} information related to masculine and feminine words.
Additionally, word analogies are used to evaluate gender bias in static embeddings \cite{Tolga:NIPS:2016,manzini-etal-2019-black,Zhao:2018ab}. 
However, the above benchmarks do not consider the sense of the word.
Therefore, it is not possible to evaluate the bias of static sense embeddings.

\newcite{loureiro2019language} showed that the gender bias is learned in static sense embeddings by showing the examples.
On the other hand, we create a benchmark for evaluating sense embeddings and perform a larger survey.


\paragraph{Contextualised Embeddings:}
\newcite{may-etal-2019-measuring} extends WEAT to sentence encoders by creating artificial sentences using templates and use cosine similarity between the sentence embeddings as the association metric.
% such as ``\emph{This is [target]}'' and ``\emph{They are [attribute]}''
\newcite{kurita-etal-2019-measuring} proposed the log-odds of the target and prior probabilities of the sentences computed by masking respectively only the target vs. both target and attribute words.
% \newcite{kurita-etal-2019-measuring} showed that cosine similarity is not suitable as an evaluation measure and proposed the log-odds of the target and prior probabilities of the sentences computed by masking respectively only the target vs. both target and attribute words.

To create human annotated contexts instead of artificial contexts, \newcite{Nadeem:2020}
created \textbf{StereoSet} benchmark and \newcite{crows-pairs} created Crowdsourced Stereotype Pairs benchmark (\textbf{CrowS-Pairs}).
These benchmarks create a sentence pair like ``\emph{She is a nurse/doctor}''.
Then StereoSet calculates log-odds by masking the modified tokens (\emph{nurse}, \emph{doctor}) of the sentence pair, whereas CrowS-Pairs calculates log-odds by masking the unmodified tokens (\emph{She}, \emph{is}, \emph{a}) of the sentence pair.
%crowdsourced, \textbf{StereoSet}, a dataset for associative contexts covering four types of stereotypical biases: race, gender, religion, and profession. 
%StereoSet contains test instance both at intrasentence and intersentence discourse levels.
% ``\emph{She is a nurse/doctor}''のような文対を作成し，
% SSは文対のmodify tokens (nurse, doctor) をmaskすることでlog-oddsを計算する．
% CPは文対のunmodify tokens (She, is, a) をmaskすることでlog-oddsを計算する．
%\newcite{crows-pairs} created Crowdsourced Stereotype Pairs benchmark (\textbf{CrowS-Pairs}) covering nine types of social biases. 
%Test instances in CrowS-Pairs consist of sentence pairs where one sentence is more stereotypical than the other.
\newcite{kaneko2021unmasking} proposed All Unmasked Likelihood (\textbf{AUL}) and AUL with Attention weights (\textbf{AULA}), which calculate log-odds by predicting all tokens in a test case given the contextualised embedding of the unmasked input.

These benchmarks have not been created with the word sense in mind.
Therefore, it is not possible to evaluate the bias for each sense.
